Exploring Human-in-the-Loop Test-Time Adaptation by Synergizing Active Learning and Model Selection

Existing test-time adaptation (TTA) approaches often adapt models with the unlabeled testing data stream. A recent attempt relaxed the assumption by introducing limited human annotation, referred to as Human-In-the-Loop Test-Time Adaptation (HILTTA) in this study. The focus of existing HILTTA studies lies in selecting the most informative samples to label, a.k.a. active learning. In this work, we are motivated by a pitfall of TTA, i.e. sensitivity to hyper-parameters, and propose to approach HILTTA by synergizing active learning and model selection. Specifically, we first select samples for human annotation (active learning) and then use the labeled data to select optimal hyper-parameters (model selection). To prevent the model selection process from overfitting to local distributions, multiple regularization techniques are employed to complement the validation objective. A sample selection strategy is further tailored by considering the balance between active learning and model selection purposes. We demonstrate on 5 TTA datasets that the proposed HILTTA approach is compatible with off-the-shelf TTA methods and such combinations substantially outperform the state-of-the-art HILTTA methods. Importantly, our proposed method can always prevent choosing the worst hyper-parameters on all off-the-shelf TTA methods. The source code is available at https://github.com/Yushu-Li/HILTTA.

==> TMLR/table_HILTTA.tex <==
\begin{table}[htbp]
% \vspace{-0.3cm}
  \centering
  
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{c|c|c|crr|crr|crr|crr}
    \toprule[1.2pt]
    \multirow{2}[2]{*}{} & \multicolumn{1}{c|}{Active} & Model  & \multicolumn{3}{c|}{\textbf{ImageNet-C}} & \multicolumn{3}{c|}{\textbf{ImageNet-D}} & \multicolumn{3}{c|}{\textbf{CIFAR100-C}} & \multicolumn{3}{c}{\textbf{CIFAR10-C}} \\
          & \multicolumn{1}{c|}{Learning} & Select. & \multicolumn{1}{c|}{Worst} & \multicolumn{1}{c|}{Avg.} & \multicolumn{1}{c|}{Best} & \multicolumn{1}{c|}{Worst} & \multicolumn{1}{c|}{Avg.} & \multicolumn{1}{c|}{Best} & \multicolumn{1}{c|}{Worst} & \multicolumn{1}{c|}{Avg.} & \multicolumn{1}{c|}{Best} & \multicolumn{1}{c|}{Worst} & \multicolumn{1}{c|}{Avg.} & \multicolumn{1}{c}{Best} \\
    \midrule
    \multicolumn{1}{c|}{\small{Source}} & \multicolumn{1}{c|}{\times} & \times & \multicolumn{3}{c|}{82.02} & \multicolumn{3}{c|}{58.98} & \multicolumn{3}{c|}{46.44} & \multicolumn{3}{c}{43.51} \\
    \midrule
    \multicolumn{1}{c|}{\small{TENT \cite{wang2020tent}}} & \multicolumn{1}{c|}{\times} & \times & \multicolumn{1}{c|}{95.23} & \multicolumn{1}{c|}{73.13} & \multicolumn{1}{c|}{62.96} & \multicolumn{1}{c|}{83.54} & \multicolumn{1}{c|}{59.82} & \multicolumn{1}{c|}{52.93} & \multicolumn{1}{c|}{94.26} & \multicolumn{1}{c|}{50.69} & \multicolumn{1}{c|}{32.75} & \multicolumn{1}{c|}{71.22} & \multicolumn{1}{c|}{27.77} & \multicolumn{1}{c}{18.14} \\
    \midrule
     & \cellcolor[rgb]{ .816,  .808,  .808} & \cellcolor[rgb]{ .816,  .808,  .808}\times & \multicolumn{1}{c|}{\cellcolor[rgb]{ .816,  .808,  .808}95.04} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .816,  .808,  .808}67.08 (\textbf{+6.05})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .816,  .808,  .808}59.60} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .816,  .808,  .808}79.15} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .816,  .808,  .808}55.01 (\textbf{+4.81})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .816,  .808,  .808}49.59} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .816,  .808,  .808}94.26} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .816,  .808,  .808}50.70 (-0.01)} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .816,  .808,  .808}30.87} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .816,  .808,  .808}64.61} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .816,  .808,  .808}24.91 (\textbf{+2.86})} & \multicolumn{1}{c}{\cellcolor[rgb]{ .816,  .808,  .808}16.84} \\
          &  \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[rgb]{ .816,  .808,  .808}Random}}      & \cellcolor[rgb]{ .816,  .808,  .808}\checkmark & \multicolumn{3}{c|}{\cellcolor[rgb]{ .816,  .808,  .808}59.42 (\textbf{+13.71})} & \multicolumn{3}{c|}{\cellcolor[rgb]{ .816,  .808,  .808}49.56 (\textbf{+10.26})} & \multicolumn{3}{c|}{\cellcolor[rgb]{ .816,  .808,  .808}31.50 (\textbf{+19.19})} & \multicolumn{3}{c}{\cellcolor[rgb]{ .816,  .808,  .808}17.80 (\textbf{+9.97})} \\
\cmidrule{2-15}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{\cellcolor[rgb]{ .886,  .937,  .855}}} & \cellcolor[rgb]{ .886,  .937,  .855}\times & \multicolumn{1}{c|}{\cellcolor[rgb]{ .886,  .937,  .855}95.23} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .886,  .937,  .855}70.47 (\textbf{+2.66})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .886,  .937,  .855}60.79} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .886,  .937,  .855}82.39} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .886,  .937,  .855}56.27 (\textbf{+3.55})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .886,  .937,  .855}49.85} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .886,  .937,  .855}94.37} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .886,  .937,  .855}51.33 (-0.64)} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .886,  .937,  .855}30.18} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .886,  .937,  .855}29.46} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .886,  .937,  .855}18.45 (\textbf{+9.32})} & \multicolumn{1}{c}{\cellcolor[rgb]{ .886,  .937,  .855}15.77} \\
          & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[rgb]{ .886,  .937,  .855}Entropy \cite{shannon1948mathematical}}}       & \cellcolor[rgb]{ .886,  .937,  .855}\checkmark & \multicolumn{3}{c|}{\cellcolor[rgb]{ .886,  .937,  .855}60.45 (\textbf{+12.68})} & \multicolumn{3}{c|}{\cellcolor[rgb]{ .886,  .937,  .855}49.48 (\textbf{+10.34})} & \multicolumn{3}{c|}{\cellcolor[rgb]{ .886,  .937,  .855}32.78 (\textbf{+17.91})} & \multicolumn{3}{c}{\cellcolor[rgb]{ .886,  .937,  .855}15.82 (\textbf{+11.95})} \\
\cmidrule{2-15}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{\cellcolor[rgb]{ .839,  .863,  .898}}} & \cellcolor[rgb]{ .839,  .863,  .898}\times & \multicolumn{1}{c|}{\cellcolor[rgb]{ .839,  .863,  .898}94.49} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .839,  .863,  .898}69.90 (\textbf{+3.23})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .839,  .863,  .898}60.73} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .839,  .863,  .898}80.15} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .839,  .863,  .898}56.40 (\textbf{+3.42})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .839,  .863,  .898}50.83} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .839,  .863,  .898}94.56} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .839,  .863,  .898}53.08 (-2.39)} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .839,  .863,  .898}32.08} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .839,  .863,  .898}60.62} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .839,  .863,  .898}25.92 (\textbf{+1.85})} & \multicolumn{1}{c}{\cellcolor[rgb]{ .839,  .863,  .898}17.81} \\
          & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[rgb]{ .839,  .863,  .898}K-Center \cite{sener2018active}}}      & \cellcolor[rgb]{ .839,  .863,  .898}\checkmark & \multicolumn{3}{c|}{\cellcolor[rgb]{ .839,  .863,  .898}60.56 (\textbf{+12.57})} & \multicolumn{3}{c|}{\cellcolor[rgb]{ .839,  .863,  .898}50.60 (\textbf{+9.22})} & \multicolumn{3}{c|}{\cellcolor[rgb]{ .839,  .863,  .898}33.25 (\textbf{+17.44})} & \multicolumn{3}{c}{\cellcolor[rgb]{ .839,  .863,  .898}17.97 (\textbf{+9.80})} \\
\cmidrule{2-15}          \small{TENT}& \cellcolor[rgb]{ .984,  .898,  .839} & \cellcolor[rgb]{ .984,  .898,  .839}\times & \multicolumn{1}{c|}{\cellcolor[rgb]{ .984,  .898,  .839}93.82} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .984,  .898,  .839}71.51 (\textbf{+1.62})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .984,  .898,  .839}62.78} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .984,  .898,  .839}79.06} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .984,  .898,  .839}54.91 (\textbf{+4.91})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .984,  .898,  .839}49.65} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .984,  .898,  .839}94.34} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .984,  .898,  .839}51.20 (-0.51)} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .984,  .898,  .839}31.59} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .984,  .898,  .839}59.06} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .984,  .898,  .839}24.41 (\textbf{+3.36})} & \multicolumn{1}{c}{\cellcolor[rgb]{ .984,  .898,  .839}17.15} \\
          \small{w/ HIL}&    \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[rgb]{ .984,  .898,  .839}VeSSAL \cite{saran2023streaming}}}    & \cellcolor[rgb]{ .984,  .898,  .839}\checkmark & \multicolumn{3}{c|}{\cellcolor[rgb]{ .984,  .898,  .839}62.37 (\textbf{+10.76})} & \multicolumn{3}{c|}{\cellcolor[rgb]{ .984,  .898,  .839}49.56 (\textbf{+10.26})} & \multicolumn{3}{c|}{\cellcolor[rgb]{ .984,  .898,  .839}32.89 (\textbf{+17.80})} & \multicolumn{3}{c}{\cellcolor[rgb]{ .984,  .898,  .839}17.81 (\textbf{+9.96})} \\
\cmidrule{2-15}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{\cellcolor[rgb]{ 1,  .949,  .8}}} & \cellcolor[rgb]{ 1,  .949,  .8}\times & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .949,  .8}93.57} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .949,  .8}68.85 (\textbf{+4.28})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .949,  .8}60.66} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .949,  .8}78.32} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .949,  .8}54.25 (\textbf{+5.57})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .949,  .8}49.35} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .949,  .8}94.35} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .949,  .8}48.19 (\textbf{+2.50})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .949,  .8}30.53} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .949,  .8}70.23} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .949,  .8}25.36 (\textbf{+2.41})} & \multicolumn{1}{c}{\cellcolor[rgb]{ 1,  .949,  .8}17.04} \\
          &    \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[rgb]{ 1,  .949,  .8}ASE \cite{kossen2022active}}}    & \cellcolor[rgb]{ 1,  .949,  .8}\checkmark & \multicolumn{3}{c|}{\cellcolor[rgb]{ 1,  .949,  .8}60.52 (\textbf{+12.61})} & \multicolumn{3}{c|}{\cellcolor[rgb]{ 1,  .949,  .8}53.08 (\textbf{+6.74})} & \multicolumn{3}{c|}{\cellcolor[rgb]{ 1,  .949,  .8}31.16 (\textbf{+17.53})} & \multicolumn{3}{c}{\cellcolor[rgb]{ 1,  .949,  .8}17.49 (\textbf{+10.28})} \\
\cmidrule{2-15}          & \multicolumn{1}{r|}{\multirow{2}[2]{*}{\cellcolor[rgb]{ .871,  .922,  .969}}} & \cellcolor[rgb]{ .871,  .922,  .969}\times & \multicolumn{1}{c|}{\cellcolor[rgb]{ .871,  .922,  .969}94.59} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .871,  .922,  .969}69.09 (\textbf{+4.04})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .871,  .922,  .969}60.71} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .871,  .922,  .969}79.99} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .871,  .922,  .969}55.25 (\textbf{+4.57})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .871,  .922,  .969}49.89} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .871,  .922,  .969}94.64} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .871,  .922,  .969}48.70 (\textbf{+1.99})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .871,  .922,  .969}30.36} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .871,  .922,  .969}31.28} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .871,  .922,  .969}19.35 (\textbf{+8.42})} & \multicolumn{1}{c}{\cellcolor[rgb]{ .871,  .922,  .969}16.39} \\
          &   \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[rgb]{ .871,  .922,  .969}SimATTA \cite{Anony2024ATTA}}}    & \cellcolor[rgb]{ .871,  .922,  .969}\checkmark & \multicolumn{3}{c|}{\cellcolor[rgb]{ .871,  .922,  .969}60.46 (\textbf{+12.67})} & \multicolumn{3}{c|}{\cellcolor[rgb]{ .871,  .922,  .969}49.59 (\textbf{+10.23})} & \multicolumn{3}{c|}{\cellcolor[rgb]{ .871,  .922,  .969}31.23 (\textbf{+19.46})} & \multicolumn{3}{c}{\cellcolor[rgb]{ .871,  .922,  .969}16.95 (\textbf{+10.82})} \\
\cmidrule{2-15}          & \cellcolor[rgb]{ 1,  .922,  1}K-Margin & \cellcolor[rgb]{ 1,  .922,  1}\times & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .922,  1}94.98} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .922,  1}68.13 (\textbf{+5.00})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .922,  1}58.49} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .922,  1}76.27} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .922,  1}53.77 (\textbf{+6.05})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .922,  1}48.55} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .922,  1}94.75} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .922,  1}49.37 (\textbf{+1.32})} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .922,  1}30.11} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .922,  1}27.81} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  .922,  1}18.21 (\textbf{+9.56})} & \multicolumn{1}{c}{\cellcolor[rgb]{ 1,  .922,  1}15.75} \\
          &    \cellcolor[rgb]{ 1,  .922,  1}(OURS)   & \cellcolor[rgb]{ 1,  .922,  1}\checkmark & \multicolumn{3}{c|}{\cellcolor[rgb]{ 1,  .922,  1}58.35 (\textbf{+14.78})} & \multicolumn{3}{c|}{\cellcolor[rgb]{ 1,  .922,  1}48.74 (\textbf{+11.08})} & \multicolumn{3}{c|}{\cellcolor[rgb]{ 1,  .922,  1}30.53 (\textbf{+20.16})} & \multicolumn{3}{c}{\cellcolor[rgb]{ 1,  .922,  1}15.87 (\textbf{+11.90})} \\
    \bottomrule[1.2pt]
    \end{tabular}}%

    % \vspace{0.1cm}

  \caption{{
  Evaluation under HILTTA with average classification error (lower is better). 'Worst', 'Avg.', and 'Best' denote the worst, average, and best performances, respectively, with the candidate hyper-parameter pool $\Omega$. The performance improvement by \textbf{Active Learning} and \textbf{Model Selection} is denoted within brackets as ($\delta$). %Furthermore, the subsequent incorporation of \textbf{Model Selection} represents an additional enhancement beyond the improvement achieved through active learning also denoted as ($\delta_2$).
 }}
 \vspace{-0.4cm}
  \label{tab:different_selection}%
\end{table}
